Safe Performance-aware Online Input Design

In this paper, we propose an input design framework for the safe online excitation and identification of uncertain linear systems without requiring informative initial data. The objective is to actively excite the system and collect sufficiently informative input-output data while maintaining safe operation and satisfactory control performance. Achieving this objective is challenging due to the potential conflict between the excitation required for learning and the safety and performance requirements, particularly when limited prior knowledge of the system is available. Inspired by the dual control principle, the proposed scheme balances exploitation for control performance with exploration for model improvement. A Bayesian learning approach is employed to update the model uncertainty online, starting from a conservative initial uncertainty set. As informative data are collected, the uncertainty set contracts, enabling progressively less conservative operation. To reduce the online computational burden, the resulting program is reformulated into a computationally tractable form. Furthermore, an online ellipsoidal terminal set with non-increasing conservatism is designed to guarantee the recursive feasibility of the proposed scheme. Numerical experiments are conducted to demonstrate the effectiveness of the proposed framework, particularly in terms of uncertainty reduction and control performance.

==> mystyleproof.tex <==
%% from here-------------------------
\makeatletter
\DeclareRobustCommand{\qed}{%
  \ifmmode % if math mode, assume display: omit penalty etc.
  \else \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \fi
  \quad\hbox{\qedsymbol}}
\newcommand{\openbox}{\leavevmode
  \hbox to.77778em{%
  \hfil\vrule
  \vbox to.675em{\hrule width.6em\vfil\hrule}%
  \vrule\hfil}}
\newcommand{\qedsymbol}{\openbox}
\newenvironment{proof}[1][\proofname]{\par
  \normalfont
  \topsep6\p@\@plus6\p@ \trivlist
  \item[\hskip\labelsep\itshape
    #1.]\ignorespaces
}{%
  \qed\endtrivlist
}
\newcommand{\proofname}{Proof}
\makeatother
%% upto here----------------------------
